DiProber: Using Dual Probing to Estimate Tor Relay Capacities in Underloaded Networks

Tor is the most popular anonymous communication network. It has millions of daily users seeking privacy while browsing the internet. It has thousands of relays to route and anonymize the source and destinations of the users packets. To create a path, Tor authorities generate a probability distribution over relays based on the estimates of the capacities of the relays. An incoming user will then sample this probability distribution and choose three relays for their paths. The estimates are based on the bandwidths of observation probes the authority assigns to each relay in the network. Thus, in order to achieve better load balancing between users, accurate estimates are necessary. Unfortunately, the currently implemented estimation algorithm generate inaccurate estimates causing the network to be under utilized and its capacities unfairly distributed between the users paths. We propose DiProber, a new relay capacity estimation algorithm. The algorithm proposes a new measurement scheme in Tor consisting of two probes per relay and uses maximum likelihood to estimate their capacities. We show that the new technique works better in the case of under-utilized networks where users tend to have very low demand on the Tor network.

==> background.tex <==
\section{Background}

\subsection{Tor}

basics of design

challenges

\subsection{History of bw measurement}

Self-advertised

TorFlow was designed to introduce an independent source of capacity measurements by having a number of \emph{bandwidth authorities} form test circuits going through each relay and measure their throughput, and use this to calculate the relay capacity. [XXX two-hop circuit, large relays] TorFlow was originally designed as a PID controller [XXX cite PID]: relays would be grouped several bins based on their current capacity value. The throughput measurement would be used to compute an \emph{error value}, which is the difference between the measured throughput of the relay and the average throughput in that bin. The intuition is that if a relay's capacity is higher than currently estimated, it will be underloaded resulting in higher measured throughput. The error value would be used to adjust the capacity using the PID update equation:

\[ c'(t) = c(t) + K_p e(t) + K_i \int_0^t e(t') dt' + K_d \rac{de(t')}{dt'} \]

The default values for the constants were $K_p = 1.0$ and $K_i = K_d = 0$, making this a simple \emph{proportional} controller. An initial experiment with this set up, however, resulted in a runaway divergence effect where the capacities of all relays continued growing without bound. As a result, TorFlow was modified to work in an \emph{adjusted capacity} mode. Here, the error value, which again was the difference between the measured bandwidth of this relay and the average bandwidth, was multiplied by the \emph{observed} bandwidth, which was the largest sustained throughput that a relay itself observed over any ten-second period over the last 5 days. In other words:

\[ c(r) = \frac{m(r)}{\sum_{r \in B} m(r') / |B|} o(r) \]

where $m(r)$ is the measured throughput of relay $r$, $B$ is the set relays in the same bin as $r$, and $o(r)$ is the observed bandwidth.



==> motivation.tex <==
\section{Problem statement and motivation \darir{needs editing}}
Considering a network of $n$ relays, currently, in order to generate the consensus file containing the capacities of the relays in the network, $n$ test paths of one relay are directed to pass through every relay in the network.The published capacity of each relay is then assumed to be equal to the bandwidth of the test path passing through it. We apply the aforementioned approach on the set relays having a capacity distribution plotted in \cref{fig:capacity}. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{capacity.pdf}
    \caption{The actual weights of the relays in the network.}
    \label{fig:capacity}
\end{figure}

At each iteration of the algorithm, we generate $N$ three relays paths, where $N$ is drawn from a random variable that follows a Poisson distribution with mean $\rate$, and where the selection of relays is done randomly weighted by the published capacities. We then find the bandwidth of the test paths, i.e. the new published capacities, using max-min bandwidth allocation algorithm. We assume that we start with a weights vector that is equal to the actual capacities vector.  The published capacities after $30$ iterations of the algorithm, and eventhough starting with the actual capacities vector, don't converge to the actual capacities, plotted in \cref{fig:estimated_consensus}. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{consensus_T20.pdf}
    \caption{The estimated weights of the relays in the network after applying the currently used algorithm.}
    \label{fig:estimated_consensus}
\end{figure}

The average error is $89\%$, while the standard deviation of the error is at $20\%$. The error is plotted in \cref{fig:consensus_error}.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{consensus_error_T20.pdf}
    \caption{The relative error after $30$ iterations of the currently used algorithm.}
    \label{fig:consensus_error}
\end{figure}


==> notations.tex <==
\paragraph*{Notations}
\label{sec:notations}
We denote the sets of reals, non-negative reals, and natural numbers by $\mathbb{R}$, $\nnreals$, and $\mathbb{N}$, respectively. We use
 $[i:j]$ to denote the interval $\{i,\,i+1,\ldots , \, j\}$ of $\mathbb{N}$, and abbreviate $[0:t]$ by $[t]$.

\sayan{We do not need any of these standard notations. Use $x >0, \geq 0$ instead of $x \in \nnreals$, etc. Introduce the $[0:t]$ notation where you use it first time.}

==> shadow.tex <==
\section{Shadow Simulations: High Fidelity Experiments}
\label{sec:shadow}

We compare the performance of $\ourmethodbrute$ and $\proptorflow$ in a simulated Tor network using Shadow~\cite{shadow}, the standard framework for simulating Tor with high fidelity. Two test networks that are one percent and three percent the size of the full Tor network respectively were configured for the simulations. The 1\% network contains 65 Tor relays (including 21 guard relays with 238 MB/s of throughput, 36 middle relays with 82 MB/s of throughput, and 8 exit relays with 97 MB/s of throughput), 500 clients, 3 directory authorities, and a bandwidth authority. The 3\% network contains 196 Tor relays (including 61 guard relays with 713 MB/s of throughput, 109 middle relays with 252 MB/s of throughput, and 26 exit relays with 359 MB/s of throughput), 2000 clients, 3 directory authorities, and a bandwidth authority.
\begin{comment}
 \nikita{what is the total bw of each class? also we have 3\% simulations, too}
\end{comment}
Each client maintains a single file download stream during a consensus round. All streams are dropped and restarted at a new consensus round to make sure that the downloads utilize circuits generated by the latest consensus. \begin{comment}
 \nikita{discuss difference b/w this and real-life Tor}
\end{comment}
We've also set the duration of each consensus round to 10 minutes to reduce the time needed to simulate each round. In real-life Tor, directory authorities generate a new consensus every hour. Clients also reuse consensus documents for up to 3 rounds. However, bandwidth authorities in the real world have a much longer refresh period. It takes several days to complete a scan of the entire Tor network.

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{mle_network.png}
    \caption{Overview of the network structure for $\ourmethodbrute$ simulation}
    \label{fig:mle_network}
\end{figure}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{mle_timeline.png}
    \caption{Execution timeline of the $\ourmethodbrute$ simulation}
    \label{fig:mle_time}
\end{figure}

For $\ourmethodbrute$, we added functionalities of the algorithm to the Tor plugin run by the directory authorities. At each consensus round, the modified directory authorities reads the measured observation of each relay from the prober (bandwidth authority) and executes the $\ourmethodbrute$ algorithm to generate published bandwidth values for all relays. Each directory authority also maintains maximum likelihood score vectors to keep track of the published bandwidth history for each relay. The matrix is updated with the scores generated from the latest observations at each round. 
%The feedback system is illustrated in figure \ref{fig:mle_network}. 
The simulation timeline is illustrated in figure \ref{fig:mle_time}. %In addition, we implemented the noise handling mechanism discussed in section \ref{noisey}. 

For $\proptorflow$, we used the latest TorFlow implementation in the Shadow Tor plugin. The plugin reimplements the logic of TorFlow in C, as Shadow does not support running Python code used to implement TorFlow 
as well as the newer sbws system. The plugin does not implement the adjusted capacity version of TorFlow, in part because it is expensive to run simulations for long periods needed to computed the relay-measured capacity. 
%For $\proptorflow$, we used the latest version of \texttt{shadow-torflow} plugin by Jansen et al. which adds the one-shot-estimation functionality to the bandwidth authority. The directory authorities simply collect the bandwidth estimations from the bandwidth authority and redistribute the results in consensus documents.


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{noise_cdf.pdf}
    \caption{CDF of noise ratios calculated using $o[j]\times (1+X[j])/C^*[j]$ for all relays $j \in [n]$ across 60 rounds of simulation. i.e. the ratio was obtained from dividing the estimated capacity (observation times \text{the number of circuits going through each relay plus one}) by the true capacity.}
    \label{fig:max_min_noises}
\end{figure}

\subsection{Estimating  Noise Ratio}

The noise-free model we use in our bandwidth estimation assumes that the bandwidth of a relay is split evenly between all the circuits going through it (including the observation circuit). In practice, this will not be the case because some of the circuits may be bottlenecked at other relays; furthermore, congestion and flow control mechanisms in Tor and TCP will cause occasional imbalance between flows. To understand this effect, we ran a simulation of the 1\% network and compared the bandwidth of the observation circuit to the bandwidth predicted by the model, i.e., the actual capacity of the relay divided by the number of circuits using the relay; i.e.,  $C^*[j] / (1+X_i[j])$. We call the ratio between these two values the \emph{noise ratio}, and we plot the ratio in Figure~\ref{fig:max_min_noises}. Figure \ref{fig:max_min_noises} shows the maximum and minimum noise ratio of all relays in each round. We can see that the noise ratio is bounded between 0.7 and 1.3 for all rounds. These numbers are used to determine the plausible range of noisy measurements for $\ourmethodbrute$.


 \begin{figure*}[h!]
    \centering
\begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{relay_entering_0.01.pdf}
    \caption{13 MB/s}
        \label{fig:relay_enter_big}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{relay_entering_small_0.01.pdf}
    \caption{3.6 MB/s}
        \label{fig:relay_enter_small}
\end{subfigure}
    \caption{Published capacities of a previously unseen relay joining the 1\% network. The target relay joins the network after 10 consensus rounds have already been simulated.}
    \label{fig:relay_enter}
\end{figure*}

\subsection{Newly Joining Relays}
Our first analysis evaluates the performance of each algorithm when a new relay joins an already-converged network. We first run both $\proptorflow$ and $\ourmethodbrute$ for 10 rounds (6000 seconds), after which a previously unseen relay joins the network. The new relay, whose true capacity is 13 MB/s, first start with zero published weight. The subsequent estimates generated by both algorithms are shown in figure \ref{fig:relay_enter_big}. For $\ourmethodbrute$, we observe that the estimation is stable and within a 10\% error after 5 consensus rounds, with the estimation inching even closer to the true capacity after 40 rounds. Meanwhile, $\proptorflow$'s estimates have larger errors throughout the simulation and shows significant fluctuations compared to $\ourmethodbrute$. We also ran the same experiemnt to estimate a previously unseen relay with a smaller capacity at 3.6 MB/s. We see similar results with this experiment where $\ourmethodbrute$ manages to maintain a stable estimate with 5\% error. Meanwhile $\proptorflow$'s fluctuates around the true capacity. The results are shown in figure \ref{fig:relay_enter_small}. %We also note that when a smaller relay with 3.5 MB/s of capacity joins the 1\% network, $\proptorflow$ could not 

\begin{figure} 
    \centering
    \centering
    \includegraphics[width=\columnwidth]{relay_avgerror_0.03.pdf}
\caption{Comparing average estimation errors of all exit relays in each round. The 3\% networks was used in this experiment.}
\label{fig:relay_avg}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{boxcompare.pdf}
    \caption{Estimation error distribution for each type of relay. Results are obtained after 22 consensus rounds in the 3\% network using Shadow.}
    \label{fig:est_error_dist}
\end{figure}

\subsection{Overall Estimation Error}
Our second analysis looks at how each algorithm performs when estimating all relays with zero initial information. That is, all relays are assumed to have equal bandwidth in the beginning. We calculate the average estimation error of all exit relays in a whole network estimation run. The results are shown in figure \ref{fig:relay_avg}. We can see that $\ourmethodbrute$ outperforms $\proptorflow$ by maintaining a low average estimation error around 10\% after running for 10 consensus rounds. $\proptorflow$, meanwhile, is only able to maintain an average error between 30\% and 50\%. The minimum achieved error by $\ourmethodbrute$ is 8\%, which is optimal considering that a 10\% quantization gap is used when configuring $\ourmethodbrute$ and is also consistent with the quantization errors shown in Table~\ref{table:low-fidelity}. We see similar results in the 3\% network, where $\ourmethodbrute$ achieved a sub 10\% average estimation error after 20 rounds compared to $\proptorflow$'s higher estimation error. The final estimation result after 22 rounds of estimation is shown in figure \ref{table:shadow_figures} in the Appendix, where the distribution of capacity estimation is categorized for each type of relay and each type of algorithm. We compare the results against the low fidelity simulation results in figure \ref{table:figures}. We see that $\ourmethodbrute$ is able to estimate the exit relays accurately in both low and high fidelity simulations. For guards and middles, $\ourmethodbrute$ is able to trace the relay distributions more closely than $\proptorflow$. Finally we aggregated the estimation error distribution for all categories of relays in \ref{fig:est_error_dist}. In all cases, $\ourmethodbrute$ achieved a lower average error with a narrower range of error.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{round_22.pdf}
    \caption{Client download bandwidth distribution after bandwidth estimation has converged.}
    \label{fig:band_dist}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{client_average.pdf}
    \includegraphics[width=0.95\columnwidth]{client_std.pdf}
    \caption{Aggregate statistics progression of client download bandwidth distribution in each consensus round. The 3\% network was used in this experiment.}
    \label{fig:band_dist_aggr}
\end{figure}


\subsection{Network Load Balancing}
Finally, we analyze the effects of $\ourmethodbrute$ and $\proptorflow$ on the bandwidth distribution across the entire network. We analyzed the results from the same 3\% whole network estimation where 2000 clients were configured to each maintain a single file download stream. Figure~\ref{fig:band_dist} shows the distribution of download speed across the 2000 clients using consensus weights generated by both $\ourmethodbrute$ and $\proptorflow$ after 22 consensus rounds. The figure shows the effects that each algorithm has on the load balancing across the entire network. Around 75\% of all clients under $\ourmethodbrute$ achieved a higher bandwidth compared to $\proptorflow$. $\ourmethodbrute$ resulted in a more even bandwidth distribution with a higher average bandwidth at 161.65 KB/s compared to $\proptorflow$'s 152.74 KB/s. The load balancing effect can also be seen in the round-to-round analysis shown in figure \ref{fig:band_dist_aggr}. For $\ourmethodbrute$, we see a smaller average bandwidth for the top performing clients, but a larger overall average and a better average for the worst performing clients compared to $\proptorflow$ in all rounds. The standard deviation of bandwidths in $\ourmethodbrute$ is also much lower than $\proptorflow$ in all rounds, which implies a fairer bandwidth allocation when using $\ourmethodbrute$.


\begin{comment}
 \begin{table*}
    \caption{Shadow simulation results after 22 consensus rounds in the 3\% network.}\label{table:high-fidelity}
    \begin{center}
        \begin{tabular}{|l|r|r|r|r|r|}
         \hline
        
            &   & \multicolumn{3}{c|}{relays cap. est. err. (\%)} & paths bw \\ \cline{3-5}
 Est. method             & stats   & guard & middle &   exit & (kb/s)\\\hline
                    &    mean &  44.33    & 78.07    & 37.81  &    152.74    \\\cline{2-6}
                    
                    &    std. &30.61      & 34.69    &  29.61 & 115.33 \\\cline{2-6}
                    
$\proptorflow$    &    max  &   173.19   &   145.35  & 99.82  &  1440.75 \\\cline{2-6}
                   
                    &    min  & 0.36     &   0.92  &  2.25 &    31.15 \\
                    
                \hline
                     &    mean &  15.37    &    41.27 & 7.98  & 161.65    \\\cline{2-6}
                    
                    &    std. & 10.33     & 20.13    &  9.8 &   31.75   \\\cline{2-6}
                    
$\ourmethodbrute$  &    max  &  40.99    &   74.52  &  38.43 &  453.91  \\\cline{2-6}
                   
                    &    min  & 0.45     &    1.41 &  0.18 & 48.21    \\
                    
                \hline
        \end{tabular}
    \end{center}
\end{table*}
\end{comment}
 

==> torflow_adjusted.tex <==
\section{Analysis of Current $\torflow$}

$\torflow$ uses two inputs to calculate a relay's capacity: the measured throughput and the observed bandwidth. In principle, the latter should be a good estimate of the fundamental bandwidth capacity of a relay, with the former creating an adjustment factor to account for erroneous or malicious observed bandwidth values. This value, however, is clearly dependent on the ``offered load'' of a relay; if, for example, few users choose the relay in their circuits, the relay may not have a chance to ``max out'' its capacity\geir{, and would consequently} report a  \geir{(potentially significantly)} lower observed value. This creates a well-known ``ramp up period'' for newly introduced relays: they are initially assigned a low weight~\cite{lifecycle-tor-relay}, which results in a low observed capacity. The throughput measurement, however, will be high since the relay is underloaded, so its published capacity will be adjusted upwards. This will cause the observed capacity to increase and gradually, over a number of measurement rounds, until the observed capacity matches the real capacity.

To better understand the dynamic of $\torflow$, we implemented a simulation using a fluid connection model. We implemented  \geir{is there more to be added, or should this be reomoved?}

\sibai{Problems with current torflow? high variance?}


==> variance.tex <==
\subsection{Variance of $\proptorflow$ $>$ Variance of $\ourmethodclosed$}
\label{sec:variance_comparison}
In this section, we show an upper bound on the variance of the estimates generated by $\ourmethodclosed$. We also present the actual variance of the estimates generated by $\proptorflow$. Furthermore, we prove that the former is upper bounded by the latter. This shows that our method $\ourmethodclosed$ provides more stable and consistent estimates compared to $\proptorflow$.
%, the currently used method.
% These variance will be used later to compare with the upper bound of the variance of our proposed method in \cref{thm:closedformsol}.
%\sibai{In the next section, we will introduce an alternative method for relays capacities estimation that is more robust to noise. (we can remove this)}


%We first find an upper bound on the variance of estimates by $\ourmethodclosed$.

%\sibai{Preserve the order of presentation in every section, Torflow then ours or the opposite?}

\begin{restatable}[$\ourmethodclosed$ variance upper bound]{theorem}{stdbound}
\label{thm:std_bound}
For any $j \in [n]$ and $t \in \mathbb{N}$, the variance of $C_{t+1}^{\mlflowexp}[j]$ is upper bounded by,
\begin{align}
    \Var[C_{t+1}^{\mlflowexp}[j]] \leq C^*[j]^2(e^{\frac{\mu_t^1[j]}{\mu_t^2[j]}})^2V[j],
\end{align}
where
\begin{align*}
V[j]& =\frac{(\mu_t^1[j])^2}{(\mu_t^2[j])^2}(\frac{\sigma_t^1[j]}{\mu_t^1[j]}-\frac{\sigma_t^2[j]}{\mu_t^2[j]})^2, \\ 
  (\sigma_t^1[j])^2 &=\sum_{i=0}^{t}(\log(\frac{\lambda_sw_i^{\mlflowexp}[j]}{\lambda_sw_i^{\mlflowexp}[j]+1})-1)^2\frac{\lambda_sw_i^{\mlflowexp}[j]}{{C^*[j]}^2}, \\
 \mu_t^1[j] &=\sum_{i=0}^{t}\frac{\lambda_sw_i^{\mlflowexp}[j]+1}{C^*[j]}\log(\frac{\lambda_sw_i^{\mlflowexp}[j]}{\lambda_sw_i^{\mlflowexp}[j]+1}), \\ 
 (\sigma_t^2[j])^2&=\sum_{i=0}^{t}\frac{\lambda_sw_i^{\mlflowexp}[j]}{C^*[j]^2}, \text{ and}  \\
\mu_t^2[j]&=\sum_{i=0}^{t}\frac{1}{C^*[j]}(\lambda_sw_i^{\mlflowexp}[j]+1).
\end{align*}

\end{restatable}


\begin{comment}
\begin{proof}
 (Sketch) You can find the full proof in the appendix. Using a first order Taylor series expansion, we can approximate the mean and variance of a function of random variables \sibai{specify which function} by evaluating the function at the means and variances of the random variables (\sibai{which random variables?}). We can also upper bound the covariance between two random variables using Cauchy-Schwarz inequality (\sibai{mention we used to upper bound which covariance}). Using \cref{eq:resW} and the approximation obtained, we find the expected value of $C_i[j]$ and an upper bound on the variance of $C_i[j]$ for any $j \in [n]$.
\end{proof}
\end{comment}


% Torflow estimates the capacities of relays using \cref{eq:capacity_estimate_last}.
%The value of the variance of $C_{t+1}^{\torflowexp}[j]$ is shown in the following lemma. 

\begin{restatable}[$\proptorflow$ variance]{theorem}{torflowExVar} \label{thm:tor_exvar}
For any $j \in [n]$ and $t \in \mathbb{N}$, the variance of $C_{t+1}^{\torflowexp}[j]$ is as follows:
 \begin{align}
\Var[C_{t+1}^{\torflowexp}[j]]&=C^*[j]^2\frac{(\lambda_sw_t^{\torflowexp}[j])^3}{(\lambda_sw_t^{\torflowexp}[j]+1)^4}.
\label{eq:tor4}
\end{align}
\end{restatable}

%Now that we have the variances of both methods, we compare them in the following theorem.
 

\begin{restatable}[Variance of $\proptorflow >$ Variance of $\ourmethodclosed$]{theorem}{variancecomparison}
\label{thm:varcomp}
For $\lambda_s$ big enough, for all $j \in [n]$, and starting with the same initial weights, $\Var[C_{1}^{\mlflowexp}[j]] = \Var[C_{1}^{\torflowexp}[j]]$ and  for $t \geq 1$,
\begin{align}
\label{eq:varMLE_geq_varTor}
\frac{\Var[C^{\torflowexp}_{t+1}[j]]}{\Var[C^{\mlflowexp}_{t+1}[j]]}> \frac{t+1}{1.96}.
\end{align}
\end{restatable}

\begin{restatable}
[Convergence of variance of $\ourmethodclosed$]{corollary}{varconvergence}
As $t \rightarrow \infty$, $\Var[C_{t}^{\mlflowexp}[j]] \rightarrow 0$.
\end{restatable}

%\sayan{This is the first proof that appears in the paper and it is also somewhat simple. Just wanted to draw your attention to this decision.}
% Var[C^M_{t+1}[j]] < Var[C^T_{t+1}[j]].
%\sayan{(1)If we have titles in [], corollaries should also be [] and not (). (2) Please use $\mathit{Var}$ and not $\Var$. (3) Saying (14) should be enough, no need to say equation (14), particularly if we are short of space. }

%\darir{\begin{enumerate}
%    \item We have that the gap increases as linear function of $t$: $\frac{Var[C^T_{t+1}[j]]}{Var[C^M_{t+1}[j]]}> \frac{t+1}{1.96}$
%    \item I checked and we can show that both variances go to zero when $\rate$ goes to infinity. And we know from theorem 4 that the expected values go to the actual capacity.
%\end{enumerate}}

Hence the variances of the MLE estimates when considering the full history of weights and measurements in $\ourmethodclosed$ are always less than the variances of the estimates found using only the last measurement as in $\proptorflow$. That is, the estimates of produced by  $\ourmethodclosed$ will be close to the actual capacities more frequently than those of $\proptorflow$. 
%The proof of this theorem can be found in the Appendix. 
We will show this experimentally using simulations in the next section.
% \darir{IMPORTANT: If we can find a theorem that says that a stochastic model using more information is at least of the same accuracy as the original model.}
